When Nash Meets Stackelberg

This article introduces a class of $Nash$ games among $Stackelberg$ players ($NASPs$), namely, a class of simultaneous non-cooperative games where the players solve sequential Stackelberg games. Specifically, each player solves a Stackelberg game where a leader optimizes a (parametrized) linear objective function subject to linear constraints while its followers solve convex quadratic problems subject to the standard optimistic assumption. Although we prove that deciding if a $NASP$ instance admits a Nash equilibrium is generally a $\Sigma^2_p$-hard decision problem, we devise two exact and computationally-efficient algorithms to compute and select Nash equilibria or certify that no equilibrium exists. We apply $NASPs$ to model the hierarchical interactions of international energy markets where climate-change aware regulators oversee the operations of profit-driven energy producers. By combining real-world data with our models, we find that Nash equilibria provide informative, and often counterintuitive, managerial insights for market regulators.

==> Resources/Computational.tex <==
\begin{table}[!ht]
\centering
\caption{Results for \emph{InstanceSetA}. } \label{tab:SummaryA}
\scriptsize

\begin{tabular}{@{}c@{\hspace{2em}}r@{\hspace{1.2em}}r@{\hspace{1.2em}}c@{\hspace{4.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}r@{\hspace{4.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}}
	\toprule
	\multicolumn{1}{l}{}   & 
	\multicolumn{3}{c}{\textbf{\textbf{}}}   & 
	\multicolumn{3}{c}{\textbf{Time (s)}} & 
	\multicolumn{2}{c}{\textbf{Wins}} & 
	\multicolumn{1}{l}{}  \\ 
	
	\multicolumn{1}{l}{}   & {\textbf{Algorithm}}  & { \textbf{ES}} & { $\hat{\theta}$} & { \textbf{EQ}} & { \textbf{NO}} & { \textbf{All}} & { \textbf{EQ}} & { \textbf{NO}} & { \textbf{Solved}} \\ \midrule
 & \emph{FE}   & -  & -     & 26.78  & 0.12 & 120.21 &  6 & 82 & 140/149  \\ \midrule
 &  & Seq & 1       & 6.18  & 0.35  & 51.33 & 3  &    0 &   145/149 \\
 &  & Seq & 3       & 16.20 & 0.18  & 55.82 & 5  &    0 &   145/149 \\
 &  & Seq & 5       & 5.85  & 0.15  & 51.08 & 3  &    0 &   145/149  \\
 &  & RSeq & 1   & 7.33  & 0.36  & 3.73 &  26 &    0 &   149/149  \\
 &  & RSeq & 3   & 10.31 & 0.18  & 53.12 & 4  &    0 &   145/149  \\
 &  & RSeq & 5   & 8.68  & 0.15  & 76.41 & 5  &    0 &   143/149  \\
 &  & Rand  & 1   & 4.80  & 0.36  & 26.60 & 8  &    0 &   147/149 \\
 &  & Rand  & 3   & 29.49 & 0.18  & 85.65 & 5  &    0 &   143/149 \\
\multirow{-10}{*}{{ \MNE}} & \multirow{-9}{*}{\emph{InnerApp}} 
 & Rand  & 5   & 21.59 & 0.15  & 58.26 & 2  &    0 &   145/149   \\ \midrule
 \PNE & \emph{FE-P} & - & -  & 6.46   & 0.12 & 328.23  & -- & --  &   122/149 \\
	& 
\end{tabular}

\end{table}


\begin{table}[!ht]
\centering
\caption{Results for \emph{InstanceSetB}.} \label{tab:SummaryB}
%\begin{threeparttable}
\scriptsize
\begin{tabular}{@{}c@{\hspace{2em}}r@{\hspace{1.2em}}r@{\hspace{1.2em}}c@{\hspace{4.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}r@{\hspace{4.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}r@{\hspace{2.0em}}}
	\toprule
	\multicolumn{1}{l}{}   & 
	\multicolumn{3}{c}{\textbf{\textbf{}}}   & 
	\multicolumn{3}{c}{\textbf{Time (s)}} & 
	\multicolumn{2}{c}{\textbf{Wins}} & 
	\multicolumn{1}{l}{}  \\ 
	
	\multicolumn{1}{l}{}   & {\textbf{Algorithm}}  & { \textbf{ES}} & { $\hat{\theta}$} & { \textbf{EQ}} & { \textbf{NO}} & { \textbf{All}} & { \textbf{EQ}} & { \textbf{NO}} & { \textbf{Solved}} \\ \midrule
	
 & \emph{FE}   & -  & -     & 260.29  & 1.12 & 1174.32 &  0 & 2 & 20/50   \\ \midrule
 &  & Seq & 1       & 39.26  & 9.64 & 672.24 &   1  &    0 &   32/50 \\
 &  & Seq & 3       & 62.66 & 3.88  & 616.25 &   1  &    0 &   34/50 \\
 &  & Seq & 5       & 24.03  & 2.83 & 733.97 &   1  &    0 &   30/50  \\
 &  & RSeq & 1   & 171.47 & 9.66 & 262.74 &   27 &    0 &   47/50  \\
 &  & RSeq & 3   & 13.85 & 3.86  & 585.27 &   4  &    0 &   34/50  \\
 &  & RSeq & 5   & 78.57  & 2.83 & 798.90 &   6  &    0 &   29/50  \\
 &  & Rand  & 1   & 34.65 & 9.65  & 497.06 &   0  &    0 &   37/50 \\
 &  & Rand  & 3   & 123.02 & 3.87 & 588.03 &   2  &    0 &   36/50 \\
\multirow{-10}{*}{{ \MNE}} & \multirow{-9}{*}{\emph{InnerApp}} 
 & Rand  & 5   & 39.18 & 2.86  & 711.77 & 4  &    0 &   41/50   \\ \midrule
 
 \PNE & \emph{FE-P} & - & -  & 7.36   & 1.12 & 1441.95  & -- & --  &   10/50 \\
	&
\end{tabular}
\end{table}

